When a Movement Becomes a Party: The 2015 Barcelona City Council Election

Barcelona en Com\'u, an emerging grassroots movement-party, won the 2015 Barcelona City Council election. This candidacy was devised by activists involved in the 15M movement in order to turn citizen outrage into political change. On the one hand, the 15M movement is based on a decentralized structure. On the other hand, political science literature postulates that parties historically develop oligarchical leadership structures. This tension motivates us to examine whether Barcelona en Com\'u preserved a decentralizated structure or adopted a conventional centralized organization. In this article we analyse the Twitter networks of the parties that ran for this election by measuring their hierarchical structure, information efficiency and social resilience. Our results show that in Barcelona en Com\'u two well-defined groups co-exist: a cluster dominated by the leader and the collective accounts, and another cluster formed by the movement activists. While the former group is highly centralized like the other major parties, the latter one stands out for its decentralized, cohesive and resilient structure.

==> structural-properties-networked/methods.tex <==
%\section{Methods}
In this study we have used methods of social network analysis for community detection, identification of relevant nodes, and measurement of the topological structure of a network.

\subsection{Community detection}

\subsubsection{Modularity}
The modularity measures the density of edges inside communities in comparison to edges between communities \cite{newman2004analysis}. Its value, between -1 and 1, is defined as:
\[
Q = \frac{1}{2m}\Sigma_{ij}\bigg[A_{ij} - \frac{k_i k_j}{2m}\bigg]\delta (c_i,c_j).
\]
Here $A_{ij}$ is the edge weight between nodes $i$ and $j$; $k_i$ and $k_j$ are the degrees of the nodes $i$ and $j$, respectively; $m$ represents the total number of edges in the graph. $c_i$; and $c_j$ are the communities of the nodes and $\delta$ is a simple delta function.

\subsubsection{Louvain Method}\label{sub:robust}

The Louvain Method is a community detection technique based on a greedy algorithm that attempts to optimize the modularity of a partition of a given network \cite{blondel2008fast}. The method follows a two-step approach. 

First, each node is assigned to its own community. Then, for each node $i$, the change in modularity is measured for moving $i$ from its own community into the community of each neighbor $j$:
\[
 \Delta Q = \bigg[ \frac{\Sigma_{in} + k_{i,in}}{2m} - \bigg(\frac{\Sigma_{tot} + k_i}{2m}\bigg)^2 \bigg]-\bigg[\frac{\Sigma_{in}}{2m} - \bigg(\frac{\Sigma_{tot}}{2m}\bigg)^2-\bigg(\frac{k_i}{2m}\bigg)^2\bigg] ,
\]
where $\Sigma_{in}$ is sum of all the weights of the intra-edges of the community where $i$ being moved into, $\Sigma_{tot}$ is the sum of all the weights of the edges to nodes of the community, $k_i$ is the degree of $i$, $k_{i,in}$ is the sum of the weights of the edges between $i$ and other nodes in the community, and $m$ is the sum of the weights of all edges in the network. Once this value is measured for all communities that $i$ is connected to, the algorithm locates $i$ into the community that produces the largest increase in modularity. If no increase is possible, $i$ remains in its original community. This process is applied iteratively until modularity can not be increase and a local maximum of modularity is achieved.

In the second step, the method groups all of the nodes from the same community and builds a new network where nodes are the communities from the previous step. Edges between nodes of the same community are represented by self-loops and edges from multiple nodes from the same community to a node of a different community are represented by weighted edges between corresponding communities. 

First and second steps are repeated until modularity can not be increased.

\paragraph{Adapted version to enhance the robustness of the largest clusters}
%\note[Y]{I would start with this}
Like most community detection methods, the Louvain method consists of a greedy algorithm and has a random component, so each execution produces a different result. To obtain robust results, avoiding dependency on a particular execution of the algorithm, we introduce the following method to identify the main clusters of the network in a stable way.

First, we run $N$ executions of the Louvain algorithm, which produce $N$ different partitions of the network into clusters.
Then we select the bigger clusters for each partition, and identify each cluster through its most representative nodes. In particular, as we expect that the main clusters will represent the political parties, we identify each cluster with the most central node corresponding to the account of a political party or of a political party leader. 
Finally, we assign to each cluster all the nodes that appear in that cluster in at least the  $1-\varepsilon$
of the partitions created, where $1-\varepsilon$ represents the confidence interval.

This procedure allows us to validate the results of the community detection algorithm, and to guarantee that all the nodes that are assigned to a cluster do actually belong to it with high confidence. 
The remaining nodes, that cannot be assigned in a stable way to any of the main clusters, are left out from all the clusters.


\subsection{Identification of relevant nodes: PageRank}

PageRank is a global characteristic of a node participation in some network and could be seen as a characteristic of node’s success and popularity \cite{Brin1998}. It is defined as a stationary distribution of a random walk on the directed graph. At each step, with probability $c$, the random walk follows a randomly chosen outgoing edge from a node, and with probability $(1-c)$ the walk starts afresh from a node chosen uniformly among all nodes. The constant c is called damping factor, and takes values between 0 and 1 (traditionally $c$=0.85). PageRank can be summarized in the following formula:

\[
PR(i) = c \sum_{j \rightarrow i} \frac{1}{d_j} PR(j) + \frac{1-c}{n},
\]

where $PR(i)$ is the PageRank of node $i$, $d_j$ is out-degree of node $j$, the sum is taken over all nodes $j$ that link to node $i$, and $n$ is the number of nodes in the network. Unlike in- and out-degree which are local characteristics, the PageRank is a global characteristic of a node. In other words, adding/removing an edge between two nodes could affect PageRank values of many nodes. 

\subsection{Network topology}

\subsubsection{In-degree distribution}
The in-degree of node $i$ is the total number of edges onto node $i$. By counting how many nodes have each in-degree value, the in-degree distribution $P(k_{in})$ is equal to the fraction of nodes in the graph with such in-degree $k_{in}$. The cumulative in-degree distribution $P(K \ge k_{in})$ represents the fraction of nodes in the graph whose in-degree is greater than or equal to $k_{in}$.

\subsubsection{In-degree Centralization}

A existing method to measure degree centralization was introduced by \cite{freeman1979centrality} and is based on two concepts: (1) how the centrality of the most central node exceeds the centrality of all other nodes and (2) setting the value as a ratio by comparing to a star network:
\[
C_{in} = \frac{\sum\limits_{i=1}^n [k^{in}_{*} - k^{in}_{i}]}{ \max \sum\limits_{i=1}^n [k^{in}_{*} - k^{in}_{i}] } ,
\]

where $k^{in}_{i}$ is the in-degree of node $i$, $k^{in}_{*}$ is the maximum in-degree of the network and $\max \sum\limits_{i=1}^n [k^{in}_{*} - k^{in}_{i}]$ is the maximum possible sum of differences for a graph with the same number of nodes (a star network).

\subsubsection{In-degree Inequality: Gini coefficient}

The Gini coefficient is a statistical metric to quantify the level of inequality given a distribution \cite{gini1912variabilita}. It was initially formulated in Economics to measure the income distribution by using the Lorenz curve. If $A$ is the area between the line corresponding perfect equality and $B$ is the area under the Lorenz curve, the Gini coefficient is equal to $A/(A+B)$. If the Lorenz curve is expressed by the function $Y = L(X)$, $B$ is calculated as follows:
\[
G = 1 -2 \int_0^1 L(X)dX
\]
In the context of network topology, the Gini coefficient can be applied to characterize the hierarchical structure of a network based on the inequality of its in-degree distribution. 

\subsubsection{Clustering coefficient}
Clustering coefficient measures the extent of nodes to clusted together by calculating the number of triangles in the network. For every node $i$ we set $N_i$ to be the neighborhood, i.e. $N_j=\{j\in V: (i,j)\in E\}$, and define the local clustering coefficient as 
\[Cl_i=\frac{2|(j,k)\in E: j,\;k\in N_j|}{k_i(k_i-1)}.\]
Then, following~\cite{watts1998collective} the clustering coefficient is just the average of the local clustering coefficients: $Cl=\sum_{i}Cl_i/n,$ where 
$n$ is the number of nodes in the network.

\subsubsection{Average path length}
The concept of average path length aims to measure the efficiency of information propagation in a social network by taking the mean value of the number of edges  along the shortest paths for all possible pairs of nodes. In more details, for every pair of nodes $i,j$ we set $d_{ij}$ to be the smallest number of steps among all directed paths between $i$ and $j$ and $d_{ij}=0$ if there is no such path. Then, the average path length is defined as follows: $l={\sum_{i\neq j}d_{ij}}/{n(n-1)}$.

\subsubsection{k-core decomposition}
The k-core of a graph is the maximal subgraph in which each vertex is adjacent, ignoring the direction of the edge, to at least k other nodes of the subgraph. A graph's node has a k-index equals to k if it belongs to the k-core but not to the (k+1)-core. Thus, a given network, we define a sub-network H induced by the subset of users C. H is a k-core of the network if and only if for every user in C: $deg_H(i) \leq k$ , and H is the maximum sub-graph which fulfils this condition. With $deg_H(i)$ we denote the degree of the node i in the sub-graph H. A user has k-index equal k if it belongs to the k-core but not to the (k+1)-core. 

In simple words, k-core decomposition starts with k = 1 and removes all nodes with degree equal to 1. The procedure is repeated iteratively until no vertices with degree 1 remain. Next, all removed nodes are assigned k-index to be 1. It continues with the same procedure for k = 2 and obtains vertices with indexes equal 2, and so on. The process stops when the last node from the network is removed at the ${k_{max}}^{th}$ step. The variable $k_{max}$ is then the maximum shell index of the graph.
